Neuro-Symbolic Evaluation of Text-to-Video Models using Formal Verification

Recent advancements in text-to-video models such as Sora, Gen-3, MovieGen, and CogVideoX are pushing the boundaries of synthetic video generation, with adoption seen in fields like robotics, autonomous driving, and entertainment. As these models become prevalent, various metrics and benchmarks have emerged to evaluate the quality of the generated videos. However, these metrics emphasize visual quality and smoothness, neglecting temporal fidelity and text-to-video alignment, which are crucial for safety-critical applications. To address this gap, we introduce NeuS-V, a novel synthetic video evaluation metric that rigorously assesses text-to-video alignment using neuro-symbolic formal verification techniques. Our approach first converts the prompt into a formally defined Temporal Logic (TL) specification and translates the generated video into an automaton representation. Then, it evaluates the text-to-video alignment by formally checking the video automaton against the TL specification. Furthermore, we present a dataset of temporally extended prompts to evaluate state-of-the-art video generation models against our benchmark. We find that NeuS-V demonstrates a higher correlation by over 5x with human evaluations when compared to existing metrics. Our evaluation further reveals that current video generation models perform poorly on these temporally complex prompts, highlighting the need for future work in improving text-to-video generation capabilities.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/scratch/av_algo_block.tex <==

% % Full-width algorithm block in two-column mode

% % \begin{figure*}[!t] % [t] for top placement in two-column
% % \centering
% {
% \begingroup
% \removelatexerror% Nullify \@latex@error
% \resizebox{0.90\linewidth}{!}{%
% \begin{minipage}{\textwidth} % Ensures the algorithm spans the entire page width
% \begin{algorithm}[H] % No need for [H] compatibility
% \DontPrintSemicolon
% \KwInput{Set of semantic scores across all frames given all atomic propositions 
% \{$C^\star = C^\star_{p_i, j} \mid p_i \in \propset, j \in \{1, 2, \dots, n\}\}$, set of atomic propositions $\propset$}
% \KwOutput{Video automaton $\va$}
% \Begin{
%     $Q \leftarrow \{q_0\}$ \tcp*{Initialize the set of states with the initial state}
%     $\lambda \leftarrow \{(q_0, \text{initial})\}$ \tcp*{Initialize the set of labels with the initial label}
%     $\delta \leftarrow \{\}$ \tcp*{Initialize the set of state transitions}
%     $Q_p \leftarrow \{q_0\}$ \tcp*{Track the set of previously visited states}
%     $n \leftarrow \frac{|C^\star|}{|\propset|}$ \tcp*{Calculate the total number of frames $n$}
    
%     \For{$j \gets 1$ \KwTo $n$}{
%         $Q_c \leftarrow \{\}$ \tcp*{Track the set of current states}
%         \For{$e_j^k \in 2^{|\propset|}$}{
%             \tcp{\( e_j^k \): unique combination of 0s and 1s for atomic propositions in \( \propset \)}
%             $\lambda(q_j^k) = \{v_1, v_2, \dots, v_{|\propset|} \mid v_i \in \{1,0\}\}$\;
%             $pr(j, k) \leftarrow 1$\;
%             \For{$v_i \in \lambda(q_j^k)$}{
%                 \If{$v_i = 1$}{
%                     $pr(j, k) \leftarrow pr(j, k) \cdot C^\star_{p_i, j}$\;
%                 }
%                 \Else{
%                     $pr(j, k) \leftarrow pr(j, k) \cdot (1 - C^\star_{p_i, j})$\;
%                 }
%             }
%             \If{$pr(j, k) > 0$}{
%                 $Q \leftarrow Q \cup \{q_j^k\}$\;
%                 $Q_c \leftarrow Q_c \cup \{q_j^k\}$\;
%                 $\lambda \leftarrow \lambda \cup \{(q_j^k, \lambda(q_j^k))\}$\;
%                 \For{$q_{j-1} \in Q_p$}{
%                     $\delta(q_{j-1}, q_j^k) \leftarrow pr(j, k)$\;
%                     $\delta \leftarrow \delta \cup \{\delta(q_{j-1}, q_j^k)\}$\;
%                 }
%             }
%         }
%         $Q_p \leftarrow Q_c$\;
%     }
%     $Q \leftarrow Q \cup \{q_{j+1}^0\}$\tcp*{Add terminal state}
%     $\lambda \leftarrow \lambda \cup \{(q_{j+1}^0, \text{terminal})\}$\;
%     \For{$q_{j-1} \in Q_p$}{
%         $\delta(q_{j-1}, q_{j+1}^0) \leftarrow 1$\;
%         $\delta \leftarrow \delta \cup \{\delta(q_{j-1}, q_{j+1}^0)\}$\;
%     }
%     $\va \leftarrow (Q, q_0, \delta, \lambda)$\tcp*{Return video automaton}
%     \Return $\va$\;
% }
% \caption{Video Automaton Generation}
% \label{alg:av_generation}
% \end{algorithm}
% \end{minipage}
% }
% \endgroup
% }
% \end{figure*}



% \begin{algorithm*}[h]
% \DontPrintSemicolon
% \KwInput{Set of semantic scores across all frames given all atomic propositions 
% \{$C^\star = C^\star_{p_i, j} \mid p_i \in \propset, j \in \{1, 2, \dots, n\}\}$, set of atomic propositions $\propset$}
% \KwOutput{Video automaton $\va$}
% \Begin{
%     $Q \leftarrow \{q_0\}$ \tcp*{Initialize the set of states with the initial state}
%     $\lambda \leftarrow \{(q_0, \text{initial})\}$ \tcp*{Initialize the set of labels with the initial label}
%     $\delta \leftarrow \{\}$ \tcp*{Initialize the set of state transitions}
%     $Q_p \leftarrow \{q_0\}$ \tcp*{Track the set of previously visited states}
%     $n \leftarrow \frac{|C^\star|}{|\propset|}$ \tcp*{Calculate the total number of frames $n$}
    
%     \For{$j \gets 1$ \KwTo $n$}{
%         $Q_c \leftarrow \{\}$ \tcp*{Track the set of current states}
%         \For{$e_j^k \in 2^{|\propset|}$}{
%             \tcp{\( e_j^k \): unique combination of 0s and 1s for atomic propositions in \( \propset \)}
%             $\lambda(q_j^k) = \{v_1, v_2, \dots, v_{|\propset|} \mid v_i \in \{1,0\}\}$\;
%             $pr(j, k) \leftarrow 1$\;
%             \For{$v_i \in \lambda(q_j^k)$}{
%                 \If{$v_i = 1$}{
%                     $pr(j, k) \leftarrow pr(j, k) \cdot C^\star_{p_i, j}$\;
%                 }
%                 \Else{XT
%                     $pr(j, k) \leftarrow pr(j, k) \cdot (1 - C^\star_{p_i, j})$\;
%                 }
%             }
%             \If{$pr(j, k) > 0$}{
%                 $Q \leftarrow Q \cup \{q_j^k\}$\;
%                 $Q_c \leftarrow Q_c \cup \{q_j^k\}$\;
%                 $\lambda \leftarrow \lambda \cup \{(q_j^k, \lambda(q_j^k))\}$\;
%                 \For{$q_{j-1} \in Q_p$}{
%                     $\delta(q_{j-1}, q_j^k) \leftarrow pr(j, k)$\;
%                     $\delta \leftarrow \delta \cup \{\delta(q_{j-1}, q_j^k)\}$\;
%                 }
%             }
%         }
%         $Q_p \leftarrow Q_c$\;
%     }
%     $Q \leftarrow Q \cup \{q_{j+1}^0\}$\tcp*{Add terminal state}
%     $\lambda \leftarrow \lambda \cup \{(q_{j+1}^0, \text{terminal})\}$\;
%     \For{$q_{j-1} \in Q_p$}{
%         $\delta(q_{j-1}, q_{j+1}^0) \leftarrow 1$\;
%         $\delta \leftarrow \delta \cup \{\delta(q_{j-1}, q_{j+1}^0)\}$\;
%     }
%     $\va \leftarrow (Q, q_0, \delta, \lambda)$\tcp*{Return video automaton}
%     \Return $\va$\;
% }
% \caption{Video Automaton Generation}
% \label{alg:av_generation}
% \end{algorithm*}


==> sec/scratch/sahil_pivot_draft.tex <==
    \pivot is built on four modes that are run sequentially: object-existence, object-action alignment, spatial-relationship, and overall-consistency. Let's introduce a working example to help assist in understanding the proposed methodology. Consider the prompt ``A person holding a hot dog is walking down to the street where  cars are next to a truck." In this, the TL specification for object-existence is $\Phi = \mathrm{person} \vee \mathrm{hotdog} \vee \mathrm{car} \vee \mathrm{truck}$. For object-action alignment, the TL specification is $\Phi = \mathrm{person\_holds\_hotdog} \vee \mathrm{person\_walks}$. For spatial-relationship, the specification is $\Phi = \mathrm{cars\_next\_to\_the\_truck}$. Finally, for overall consistency, the specification is $\mathrm{person\_holds\_hotdog} \vee \mathrm{person\_walks} \vee \mathrm{car\_next\_to\_truck}$.

        Each module provides optimized prompts and examples to the algorithm to maximize accuracy.
    uses a few-shot model for each module. Each model is initially trained with a small amount of data and then improved in a bootstrapping process over two stages. Both modules utilize a large language model (LLM), specifically GPT-4o, to facilitate an effective text conversion to the specification. Given the text prompt $T$ and the evaluation mode $m \in M$, where $M=$ \{\text{object existence}, \text{spatial relationship}, \text{object action alignment}, \text{overall consistency}\}.


    



    
    \pivot is defined as a two-shot algorithm with a bootstrapped fewshot model for each module. Both modules utilize LLMs, specifically GPT-4o, to facilitate an effective conversion. 
    \begin{enumerate}
        \item \textbf{Module $\alpha$: \texttt{f\_l2p}}: Module $\alpha$ takes a set of $\mathcal{N}$ examples of natural language and proposition pairings, defined as $\mathcal{D}_{train|\alpha} = \{(\mathcal{L}_i \rightarrow \mathcal{P}_i\}_{i=1}^{\mathcal{N}}$ where $\mathcal{D}_{train|\alpha} \subset \mathcal{D}_{train}$. By providing these pairings to an LLM, \texttt{f\_l2p} can effectively extract a list of propositions from natural language.
        $$\alpha_i = \texttt{f\_l2p.train}(\alpha_{i-1}, x, y, \theta_{llm})$$
        \item \textbf{Module $\beta$: \texttt{f\_lp2tl}}: Module $\beta$ takes in a set of $\mathcal{N}$ examples of natural language and propositional pairings combined with TL specifications, defined as $\mathcal{D}_{train|\beta} = \{(\mathcal{L}_i, \mathcal{P}_i \rightarrow \Phi_i\}_{i=1}^{\mathcal{N}}$ where $\mathcal{D}_{train|\beta} \subset \mathcal{D}_{train}$. This data is provided to an LLM as a list of examples, and through this, \texttt{f\_lp2tl} is able to generate TL specifications. Multiple checks are made through this process to ensure that the LLM is not hallucinating and all propositions are elements of the TL specification.
        $$\beta_i = \texttt{f\_lp2tl.train}(\beta_{i-1}, x, y, \theta_{llm})$$
    \end{enumerate}
    Both modules begin with $\alpha_0$ and $\beta_0$ and are trained $\forall i \in {0, 1, 2, ..., \mathcal{N}}$, allowing the module to incorporate all examples of the training set in its inference. 
    
    In order to formally guarantee that the $\mathcal{N}$ fewshot examples in the dataset $\mathcal{D}_{train}$ are sufficient in maximizing the accuracy of the modules, we employ MIPROv2 \cite{opsahlong2024optimizinginstructionsdemonstrationsmultistage} with DSPy \cite{khattab2023dspycompilingdeclarativelanguage}. 
    
    We first begin with a larger dataset, $\mathcal{D}$ where for module A, $\mathcal{D}_{i|\alpha} = \{\mathcal{L}_i \rightarrow \mathcal{P}_i\}$ and for module B, $\mathcal{D}_{i|\beta} = \{\mathcal{L}_i, \mathcal{P}_i \rightarrow \Phi_i\}$. We then create a bootstrapped dataset from $\mathcal{D}$ defined as $\mathcal{D}'$. This dataset solely comprises of effective few-shot examples via approaches based on rejection-sampling. Different instruction candidates are generated and proposed using an LLM depending on the parameters in $\theta_{llm}$, yielding the instruction set $x_{llm} = \{x_j\}_{j=0}^k$. Thus, given at a particular dataset entry $i$ and instruction $j$, $P_{i, j}^{pred} = \texttt{LLM}(\mathcal{L}_i, x_{j|\alpha}, \theta_{llm})$ for module $\alpha$, and $\Phi_{i, j}^{pred} = \texttt{LLM}(\mathcal{L}_i, \mathcal{P}_i, x_{j|\beta}, \theta_{llm})$ for module $\beta$.

    Accuracy functions are now defined; for module $\alpha$, $f_\alpha(\mathcal{D}, i, j) = \pi(\mathcal{P}_i, \mathcal{P}_{i, j}^{pred})$ and for module $\beta$, $f_\beta(\mathcal{D}, i, j) = \pi(\Phi_i, \Phi_{i, j}^{pred})$. 

    
    Bayesian Optimization is then used, creating an optimal subset, $\mathcal{D}_{train}$ of size $\mathcal{N}$ with the following operation:
    $$\mathcal{D}_{train|\alpha} = \arg\max_{\mathcal{D}_s \subset \mathcal{D}_\alpha', |\mathcal{D}_s| = \mathcal{N}} \mathbb{E}[\sum_{i \in \mathcal{D}_s} \max_{0 \leq j \leq k} f_\alpha(\mathcal{D}_s, i, j)]$$
    $$\mathcal{D}_{train|\beta} = \arg\max_{\mathcal{D}_s \subset \mathcal{D}_\beta', |\mathcal{D}_s| = \mathcal{N}} \mathbb{E}[\sum_{i \in \mathcal{D}_s} \max_{0 \leq j \leq k} f_\beta(\mathcal{D}_s, i, j)]$$


==> sec/scratch/scratch.tex <==
% Video generation technologies have had a profound impact on diverse industry sectors, opening a new era of media production across music, entertainment, advertisement, and more. Major companies are now competing to leverage these generative modes for creating advertisements, aiming to reduce advertisement costs. Furthermore, the growing demand for synthetic video in training and testing deep neural networks necessitates robust evaluation methods for synthetic or generated video. While state-of-the-art video evaluation methods provide tools to assess the video generative models, they are limited to evaluating the video at the semantic level, missing a significant component: the temporal aspect. Additionally, some of these evaluation metrics rely on basic counting and filtering functions, lacking the rigor of formal evaluation methods. Hence, we propose a novel evaluation method that combines temporal logic specifications and formal verification techniques with video foundation models. Our method introduces a more rigorous, structured framework for assessing video generative models, capturing both semantic and temporal dimensions.


% Imagine we need to retrain a model to perform in an unseen or failed scenario such as a ``A car is trying to change lanes, but a car behind in the target lane starts accelerating, so it returns to its original lane'' for a safety-critical application in autonomous driving (AD) systems. Suppose we generate the desired synthetic AD video using a text-to-video (T2V) model. If we use the unverified synthetic AD video data to retrain an AD model, the AD model's performance might degrade and can lead to catastrophic accidents. For instance, in this driving scenario, we must ensure that the synthetic video includes the car returning to its original lane only when the car behind the target lane suddenly accelerates. To evaluate the adherence of the synthetic video to the text prompt, we need a robust evaluation metric which can accurately capture the temporal evolution of events such as ``car returning to its lane'' and ``car in the target lane accelerating'' over time. If the synthetic driving video, for example, shows the car returning to its original lane midway through a lane change --- either because the car behind is too far away or for no discernible reason --- this could mislead the autonomous driving (AD) model during retraining, potentially causing it to make incorrect decisions in critical situations. Therefore, we need an evaluation method that rigorously assesses how faithfully the generated video adheres to the specific details and conditions described in the text prompt. These metrics are crucial for ensuring that synthetic data used in retraining does not introduce harmful errors into safety-critical systems like autonomous driving.
% Therefore, it is essential to develop an evaluation method that rigorously assesses two key aspects of T2V models: 1) \textbf{temporal fidelity}, which ensures that the sequence of events unfolds in a logically consistent and time-accurate manner, and 2) \textbf{T2V alignment accuracy}, which measures how faithfully the generated video adheres to the specific details and conditions described in the text prompt. These metrics are crucial for ensuring that synthetic data used in retraining does not introduce harmful errors into safety-critical systems like autonomous driving.


% Imagine we need to retrain an autonomous driving (AD) model to handle an unseen or failed scenario, such as when a car attempts to change lanes, but another car behind in the target lane accelerates, causing the first car to return to its original lane. The use of text-to-video (T2V) generative models to generate synthetic data for subsequent model retraining in a safety-critical setting such as AD presents both opportunities and risks. Therefore, we must ensure that such videos accurately reflect the intended scenario. Otherwise, unverified synthetic data, such as in the AD example, could degrade the model's performance and lead to catastrophic accidents. For instance, in this scenario, it is crucial that the synthetic video accurately depicts the car returning to its original lane only when the car behind suddenly accelerates if the video shows the car returning prematurely—either because the car behind is too far away or for no discernible reason—this could mislead the AD model during retraining, leading to incorrect decisions in real-world critical situations.

% Imagine we need to retrain an autonomous driving (AD) model to handle unseen or failed scenarios, such as aborting a lane change when a vehicle speeds in the target lane.  With recent developments in text-to-video (T2V) generative models, generating synthetic videos for such examples to retrain models for safety-critical applications like AD, offers great promise. However, if the generated videos are unverified, as in the AD example, they could degrade the model’s performance and lead to catastrophic accidents. In this particular scenario, the synthetic video must precisely depict the car returning to its original lane only when the car behind suddenly accelerates. If the video shows the car returning prematurely—whether because the car behind is too far away or for no discernible reason—this could mislead the AD model during retraining, resulting in incorrect decisions in real-world critical situations.   Therefore,  we need evaluation metrics that can rigorously assess how faithfully the generated video adheres to the specific details of the text prompt to verify synthetic videos robustly. These metrics must capture the temporal evolution of key events like ``the car returning to its lane" and ``the car in the target lane accelerating."  Consequently, evaluation methods must measure visual fidelity and reflect the accuracy of spatiotemporal relationships and temporal coherence of event sequences in the generated video.


% Our method introduces a rigorous and structured framework for assessing T2V models, capturing both semantic and spatiotemporal dimensions. 
% combines temporal logic specifications and formal verification techniques with video foundation models.

% Our method introduces a more rigorous and structured framework for assessing T2V models, capturing semantic and spatiotemporal dimensions. By incorporating temporal logic, we can formally specify and verify the temporal properties of video content, ensuring that the generated sequences adhere to the intended temporal patterns and event orderings.


%   Our method not only provides a more rigorous evaluation framework but also serves as a tool for improving the temporal coherence in generated videos. By applying formal verification techniques, we can systematically rectify temporal inconsistencies in video generation models.



% First, they lack a rigorous evaluation of event sequencing, making it difficult to determine whether the generated video adheres to the temporal order of the prompted events. Second, by operating on a per-frame basis and merely aggregating results, they fail to capture the dynamic elements that evolve across scenes. As a result, these methods do not adequately account for both spatial consistency and temporal fidelity. Therefore, there is a pressing need for sound evaluation techniques that can effectively capture both spatial consistency and temporal fidelity by analyzing the continuous evolution of dynamic elements across frames, ensuring that the generated video accurately reflects the intended sequence of events and their causal relationships over time as described in the accompanying text prompt.


% One category of approaches \citep{chivileva2023measuring} uses a video captioning model to generate a caption from the output video, which is then compared to the original prompt. Another set of approaches \citep{sun2024t2v, wu2024towards} involve transforming the prompt into a series of visual question-answering pairs (VQA) and a vision-language model (VLM) scores each frame against these pairs, which are then aggregated. 

% Finally, there are ensemble-based metrics \citep{liu2024fetv, liu2024evalcrafter, huang2024vbench} that focus primarily on visual quality, assessing aspects such as subject existence, attributes, motion consistency, and smoothness. 

% Surprisingly, despite the significant advancements in T2V models due to the evolution of diffusion-based neural video synthesis \citep{ho2020denoising, esser2023structure, blattmann2023align, zhang2023i2vgen}, robust and comprehensive methods for evaluating them remain underdeveloped. With these models being increasingly applied across a wide range of fields \citep{chen2024overview, xie2024towards,yang2015robot,xu2023controllable,wu2023unleashing,escontrela2024video,fang2022cognitive,wang2023drivedreamer,li2023drivingdiffusion}, 

% Although these methods provide visual quality, motion consistency, and semantic evaluation, they still miss critical spatiotemporal aspects that are intrinsic to video data. Specifically, they overlook two crucial factors (See \cref{fig:teaser}). First, they lack a rigorous evaluation of event sequencing, making it difficult to determine whether the generated video adheres to the temporal order of the prompted events. Second, by operating on a per-frame basis and merely aggregating results, they fail to capture the dynamic elements that evolve across scenes. As a result, these methods do not adequately account for both spatial consistency and temporal fidelity. Therefore, there is a pressing need for sound evaluation techniques that can effectively capture both spatial consistency and temporal fidelity by analyzing the continuous evolution of dynamic elements across frames, ensuring that the generated video accurately reflects the intended sequence of events and their causal relationships over time as described in the accompanying text prompt.

% \sps{TDB after we have a teaser figure --- very concisely.}
% To illustrate the limitations of current metrics, \Cref{fig:teaser} presents a video generated by Gen-3 for the prompt ``TBD LONG PROMPT WITH SEQUENCE OF EVENTS". Despite missing key elements specified in the prompt—particularly ``SUBSEQUENCE OF ORIGINAL PROMPT" -- the video is still rated highly by VBench \citep{huang2024vbench}, a widely adopted generative video evaluation metric. This discrepancy highlights how even state-of-the-art metrics can fail to accurately assess temporal fidelity and prompt alignment, underscoring the need for more robust evaluation methods.



% Moreover, we identify key limitations in existing text-to-video models—both single-shot and multi-shot—which are dominated by simplistic camera movements (e.g., zooms and pans) rather than actual temporal activities \citep{singer2022make, ho2022video}. Many of these models employ similar architectural techniques that do not capture genuine temporal dynamics, highlighting the unsolved nature of temporality in text-to-video generation. The lack of genuine temporal activities results in videos that may appear visually appealing but lack narrative coherence and temporal logic.

% \begin{itemize}
%     \item \textbf{Novel Temporal Metric}: We propose a new evaluation metric for text-to-video generation models that formally emphasizes the temporal presence and consistency of prompted events. This metric addresses the gaps in current evaluation methods that overlook temporality, providing a more comprehensive assessment of generated videos.
%     \item \textbf{Identification of Temporal Evaluation Gaps}: We analyze existing text-to-video models and highlight their key limitations in capturing temporal dynamics. By identifying the dominance of simplistic camera movements over actual temporal activities, we underscore the unsolved nature of temporality in text-to-video generation.
%     \item \textbf{Benchmark and Workflow}: We contribute a benchmark of prompts designed to test temporal properties, a new evaluation metric, and a prompting workflow that extends any existing text-to-video model for generating longer videos. This workflow enhances the temporal dynamics and properties of generated videos, leading to improved performance on our metric and paving the way for future research on long-horizon video generation.
% \end{itemize}


% Existing evaluation methods for video generation models are focused on reconstruction evaluation, which measures how closely a generated video resembles a ground-truth reference \mk{SS: Cite for the statement}. 
% These developments have resulted in both closed-source, proprietary systems like Sora \citep{videoworldsimulators2024}, Kling \citep{}, Pika \citep{}, and Gen-2, Gen-3 \citep{} \sps{fix citations}, as well as open-source models such as Open-Sora \citep{opensora}, T2V-Turbo-v2 \citep{li2024t2v}, CogVideoX \citep{hong2022cogvideo, yang2024cogvideox}, VideoCrafter2 \citep{chen2024videocrafter2}, and ModelScope \citep{wang2023modelscope}. 
% Proprietary models typically leverage vast computational power and access to exclusive datasets curated by humans, while open source models use publicly available datasets such as WebVid-10M \citep{bain2021frozen}, Panda-70M \citep{chen2024panda}, OpenVid-1M \citep{nan2024openvid}.


% - Current landscape of AI generated videos
%     - These are all of the current models that we have
%     - These are the applications that we are using them in
%     - As you see, these are mostly safety critical applications
% - Current methods to evaluate generated videos (make this match related works later)
%     - Therefore its important to ensure that the generated videos match the prompt
%     - There are a few different works that do this right now - these are the main categories of metrics/benchmarks
% - They miss the "prompt-to-video" correspondence
% - Failure of current text-to-video for temporally extended prompts
% - Our motivations, mini methodology and all the other things we are proposing in short
% - Contribution bullets

% - critical applications of text to videomodels \citep{cho2024sora}
%     - modeling: physics engine free games and VR \citep{chen2024overview}, animated texture and motion \citep{xie2024towards}
%     - Metaverse simulation
%     - robotics: robots learn from videos \citep{yang2015robot}, trajectory learning from detailed text description of movement and robotic states \citep{xu2023controllable, wu2023unleashing}, reward modelling with video generation \citep{escontrela2024video}
%     - autonomous driving: generating rare cases such as accidents \citep{fang2022cognitive}, augmentation in the real world \citep{wang2023drivedreamer}, panaromic and multi view video generation \citep{li2023drivingdiffusion}
%     - marketing: product commercials and marketing, news broadcasts, business presentations, employee orientation, news broadcasts
%     - creative uses: animation and film making, many now seen, demos have been shown by RunwayML and lots of youtube videos
%     - education: lectures to video \citep{adetayo2024text}
%     - healthcare: medical training videos, simulation of scans such as CT scans and endoscopy \citep{li2024endora, hamamci2023generatect}    
% \citep{cho2024sora} \mk{@SS can you find more citation?} \sps{I have some referneces in the comments above}, which makes accurate prompt-to-video alignment essential. 

% Applications include modeling for physics-engine-free games and virtual environments \citep{chen2024overview}, animated texture and motion \citep{xie2024towards}, in robotics for learning manipulation actions and trajectories \citep{yang2015robot, xu2023controllable, wu2023unleashing}, reward modeling with video generation \citep{escontrela2024video}, and in autonomous driving scenarios requiring rare event generation \citep{fang2022cognitive} in the real world \citep{wang2023drivedreamer}, and multi-view driving video generation \citep{li2023drivingdiffusion}. In healthcare, T2V models are also used for medical training and simulations \citep{li2024endora, hamamci2023generatect}. 

% Beyond these technical applications, these models are also being used in marketing for product commercials, news broadcasts, and business presentations. They have found creative uses in animation and filmmaking, and in education by transforming lecture notes into course videos \citep{adetayo2024text}. 

% - since we now have many applications and many models to use across them, people have been developing metrics for it
% - there are three main kind of metrics
%     - from the generated video, use a video captioning model to generate a caption and measure similarity against original prompt for video generation
%     - convert the prompt to a list of VQA pairs which a VLM scores each video frame on and then aggregated
%     - an ensemble of visual quality metrics about the subjects, their attributes, motion quality and smoothness

% \sps{Might consider only mentioning the last type of approaches to shorten introduction, other ones can stay in related works}
% \sps{Add more references to first two approaches/refactor based on related works}


% Although these methods provide valuable insights, they often lack any mechanisms to actually capture the temporal alignment of events described in the prompt, a gap our proposed metric aims to address.

% - but something missing in all of these methods is that, first the sequencing of events is not rigorously measured. and secondly, they operate in a per-frame basis and then aggregate over all frames which does not seem like a good idea where there are many dynamic elements in the scene 

% However, these methods overlook two critical aspects. First, they lack a rigorous evaluation of event sequencing, making it difficult to assess whether the video follows the temporal order of prompted events. Second, by operating on a per-frame basis and aggregating results, they fail to capture the dynamic elements that evolve across scenes.

% \sps{If we're considering removal of existing approaches from above to shorten intro, could consider merging applications and impact of low-quality videos on applications into a single parah}
% When generating a video from a prompt, users expect not only visual consistency but also faithfulness to the intended nature and sequence of events, especially for temporally extended scenarios. 
% The importance of this alignment is evident when considering the impact on the applications themselves, as discussed earlier. In safety-critical fields such as autonomous driving or healthcare training, inaccuracies in event sequencing or dynamic consistency can lead to severe consequences, such as misrepresentation of rare driving scenarios or procedural errors in medical simulations. 
% This gap in temporal coherence measurement is a key motivation for our proposed method, which directly evaluates the temporal structure and alignment of events within the generated video. 

% Such gaps in alignment may not only impair usability, but could also pose serious risks, highlighting the urgent need for metrics that rigorously evaluate prompt-to-video alignment in these models.

% Text-to-video models are increasingly being applied across a wide range of fields, making accurate prompt-to-video alignment essential. When generating a video from a prompt, users expect not only visual consistency but also faithfulness to the intended nature and sequence of events, especially for temporally extended scenarios. However, current methods for evaluating generated videos often place disproportionate emphasis on aesthetic quality, such as visual appeal and smoothness of motion, while neglecting crucial aspects like prompt fidelity and temporal alignment. This aesthetic focus can lead to misleading evaluations, especially in scenarios where sequential correctness and event-level accuracy are far more important than purely visual quality.

% Despite substantial advancements in video generative models, evaluating the quality and reliability of generated videos remains a challenging task. State-of-the-art video evaluation methods primarily assess videos at the \emph{semantic} level, focusing on aspects such as image quality, content relevance, and aesthetic appeal \citep{wu2022tune, zhu2022disco}. While these methods provide valuable insights, they often overlook a critical component of video content: the \emph{temporal} aspect. Temporal dynamics are fundamental to the coherence and realism of video sequences, influencing how events unfold over time and how viewers perceive motion and action within the video.

% Existing evaluation metrics tend to rely on basic counting and filtering functions, lacking the rigor of formal evaluation methods \citep{yan2023videogpt}. This limitation is particularly pronounced in text-to-video generation models, where capturing temporal consistency and the correct sequencing of events is crucial. Current metrics, such as VBench \citep{huang2024vbench}, predominantly focus on aesthetic quality and fail to adequately assess the temporal presence and consistency of prompted events.

% Novel Temporal Metric: We propose a novel evaluation metric for text-to-video generation models that “formally” emphasizes the temporal presence and consistency of prompted events, addressing gaps in current metrics that overlook temporality (VBench, etc. which predominantly focuses on aesthetic quality).
% Temporal Evaluation Gaps: We identify key limitations in existing text-to-video models—both single-shot and multi-shot—which are dominated by simplistic camera movements (e.g., zooms and pans) rather than actual temporal activities. Existing research often employs similar techniques at an architectural level, lacking genuine temporal dynamics. We highlight the unsolved nature of temporality for Text-to-Video.
% Benchmark and Workflow: We contribute a benchmark of prompts, a new evaluation metric, and a prompting workflow that extends any existing text-to-video model for generating longer videos. This workflow extends the temporal dynamics and properties of these generated videos and leads to improved performance on our metric, paving the way for future research on long-horizon video generation.


% In our proposed methodology, we construct a video automaton with the DTMC to formally represent the generated video and compute the final evaluation score via the formal method. The final score reflects a semantic evaluation of each atomic proposition satisfaction probability of the TL specification with

% It consists of two modules: a text-to-proposition module $\ttp : T \times M \xrightarrow{\theta^\star} \propset$ and a text-to-TL specification module $\tttl : T \times \propset \times M \xrightarrow{\theta^\star} \spec$, where $\theta^\star$ is an optimized prompt or selected few-shot examples as illustrated in .

% where $(t_1,\dots,t_k)$ is the sequence of tokens in the response. Each term $P(t_j | \cdot)$ for the token $t_j$ corresponds to the value after the softmax over the logits $e^{l_{j,.}}$, hence $P(t_j | \cdot) = \frac{e^{l_{j,\mathbf{1}_{k=t_j}}}}{\sum_{z}e^{l_{j,z}}}.$ Here, $\mathbf{1}_{k=t_j}$ indicates the position $k$ in the logit vector corresponding to the token $t_j$. We present the prompt for the semantic detector VLM in the Appendix.


% To establish a baseline, we utilize the prompt set provided by VBench, a widely recognized standard for the evaluation of generated videos. In addition, we introduce a custom prompt suite, specifically crafted to contain temporally informative prompts that rigorously test each model’s ability to maintain temporal coherence and accurately reflect event sequences. We obtain human preference labels using Amazon Mechanical Turk. 
% \sps{Do we include benchmark statistics here, or in \Cref{sec:final-benchmark}? We also open-source our benchmark and prompts.} \mk{We should mention that we make our benchmark and prompts open to the public.}

% Building upon the experimental setup, we now focus on the empirical evaluation of \neusv{}. As mentioned earlier in \Cref{sec:experiment}, we benchmark a combination of two state-of-the-art closed-source models and open-source models, namely Gen-3 and Pika, and T2V-Turbo-v2 \citep{li2024t2v} and CogVideoX-5B \citep{yang2024cogvideox} respectively. Through our experiments, we aim to address three key questions central to evaluating our approach. 

% - as mentioned earlier, we use a combination of two closed source models (Gen-3 and Pika) and two open source models (CogVideoX and T2V-Turbo-v2) for our evaluation
% - we generate videos for each of these models first based on the prompts from the vbench benchmark and then based on our own prompt set
% - the results are present in the following table
% - we also include correspondence to human scores for both visual and prompt-to-video alignment scores
% - we see that the alignment of vbench scores with human scores are lower but \neusv with human preference labels are higher
% - this is even more prominent in our prompt suite as it focuses more on temporally extended prompts

% As mentioned earlier, in our evaluation, we use a combination of two closed-source models (Gen-3 and Pika), and two open-source models (T2V-Turbo-v2 \citep{li2024t2v} and CogVideoX-5B \citep{yang2024cogvideox}). Videos are generated for each model using both the VBench benchmark prompts and our custom prompt suite. The results are summarized in the following table, where we present the alignment scores with human evaluations for both visual fidelity and prompt-to-video correspondence. Our findings indicate that while VBench scores show lower alignment with human judgments, our proposed method, \neusv, achieves significantly higher correspondence with human preference labels especially for the semantic score. This improvement is particularly pronounced with our prompt suite, which challenges the models' ability to handle temporal structure, empasizing the effectiveness of \neusv in scenarios requiring extended temporal fidelity.

% - we evaluate these video generation models using both \neusv and VBench, one of the well establish visual quality based benchmark
% - we plot these against human scores on text-to-video alignment to see how they are correlated in \Cref{fig:human-corr-vbench-neusv} 
% - across all video generation models, we find that \neusv{} consistently shows stronger correlation with human annotations in terms of the best fit line and pearson coefficient as compared to vbench
% - By incorporating temporal logic, we can formally specify and verify the temporal properties of video content, ensuring that the generated sequences adhere to the intended temporal patterns and event orderings.

% enables formal specification and verification of temporal properties within video content, measuring if these generated sequences adhere to intended event orderings.
% - now we break down and analyze the performance of each of the Text-to-Video models on our evaluation suite
% - \Cref{results-our-dataset} shows this break down by theme and by complexity
% - we find that most of these models are stronger at generating videos of nature, human and animal activities
% - the Gen-3 model scores highest across the whole suite, also confirmed by most human annotators
% - \Cref{modes-of-temporal-logic} shows how each of the four temporal specification modes of \ourpivot are distributed for the models
% - different prompts seem to rely on different modes, thereby a combination of these modes comprehensively covers most things prompts tend to specify

% - Can we empirically measure prompt coverage with TL breakdown vs with LLM
% - there are a few methods which use an LLM to compose a set of questions given a prompt
% - through this first ablation, we try to see if using temporal logic specification provides any edge over just using an LLM both in terms of human correspondence as well as with respect to coverage on the original prompt
% - Ablation w/ w/o video-to-automata: we also remove the automata construction, and rather just use a VLM and aggregate scores frame-wise as other methods do. similarly we measure human corresnpondence on this
% - through the TL ablation, we find that although the prompts generated by the LLM have good coverage, they still do not have strong correlation as since they operate on a per-frame basis on simple VQA questions, they fail to capture long term dependencies which are otherwise captured through the temporal specificiation
% - ablation without automata also shows lower correspondence highlighting that its important
% To understand the impact of temporal logic (TL) specifications on prompt coverage and human correspondence, we perform a couple of ablation studies. First, we compare TL-based prompt coverage with an alternative approach using an LLM to generate a set of questions based on the prompt. This ablation examines whether temporal logic specifications offer an advantage over LLM-generated questions, both in terms of alignment with human evaluations and coverage of the original prompt. This mimics some of the approaches such as \citept{sun2024t2v, wu2024towards}. Next, we perform an ablation by removing the video-to-automata construction and instead directly use a VLM to score each frame independently, aggregating scores frame-by-frame, similar to existing methods \citept{huang2024vbench} and \citept{liu2024evalcrafter}. We then assess human correspondence for this approach as well.

% Our findings reveal that while the LLM-generated prompts achieve reasonable prompt coverage, they lack strong correlation with human evaluations, as they operate on a per-frame basis using simple VQA questions and thus fail to capture long-term dependencies. In contrast, TL specifications are able to incorporate these dependencies. Similarly, the ablation without automata construction shows lower correspondence with human evaluations, highlighting the importance of both temporal specification and automata-based evaluation for achieving robust prompt-to-video alignment.


% plotting the density of scores on the aligned and misaligned pairs. Our results show that \neusv{} successfully separates the positive and negative sets, assigning higher scores to aligned pairs and lower scores to misaligned ones. In contrast, VBench is weaker to differentiate these sets effectively, highlighting \neusv{}'s ability to capture meaningful text-to-video alignment.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth, height=1in, draft]{assets/msr-vtt-density-neusv.pdf}
%     % \includegraphics[width=\linewidth]{assets/msr-vtt-density.pdf}
%     \caption{MSR VTT Density Plots}
%     \label{fig:msr-vtt-density}
% \end{figure}

% \sps{LLaMa 3.2 Vision vs InterVL and Multi Frame vs Single Frame}
% \lipsum[1]

% - in this first ablation of architectural choices, we see if more frames are necessarily better for \neusv{}
% - to measure this, we try using a single frame and three frames when prompting our VLM (InternVL2-8B)
% - as seen in \Cref{ablation-number-of-frames}, using 3 frames seems to offer consistently higher correlation with text-to-video alignment annotations
% - we do not try stacking more frames as it ends up exceeding the context window of the LLM

% - in this second ablation, we see if the VLM that we choose makes a difference in automata construction
% - we use two recent VLMs, the InternVL2-8B and LLaMa3.2-11B-Vision models
% - as seen in \Cref{ablation-choice-of-vlm}, internvl2-8b offers seems to offer consistently higher correlation with text-to-video alignment annotations
% - this might be because we had trouble calibrating LLaMa3.2 model as it was being overconfident with its outputs

% This raises a fundamental question about their capabilities: Are these models genuinely translating text to video, or are they merely generating visually pleasing sequences without temporal fidelity?


% To address this, we introduce \neusv{}, a novel metric that translates prompts to temporal logic specification and the automaton representation of synthetic videos, \neusv{} offers rigorous evaluations on text-to-video alignment. 
